Seeing is Believing: Rich-Context Hallucination Detection for MLLMs via Backward Visual Grounding

Multimodal Large Language Models (MLLMs) have unlocked powerful cross-modal capabilities, but still significantly suffer from hallucinations. As such, accurate detection of hallucinations in MLLMs is imperative for ensuring their reliability in practical applications. To this end, guided by the principle of "Seeing is Believing", we introduce VBackChecker, a novel reference-free hallucination detection framework that verifies the consistency of MLLMgenerated responses with visual inputs, by leveraging a pixellevel Grounding LLM equipped with reasoning and referring segmentation capabilities. This reference-free framework not only effectively handles rich-context scenarios, but also offers interpretability. To facilitate this, an innovative pipeline is accordingly designed for generating instruction-tuning data (R-Instruct), featuring rich-context descriptions, grounding masks, and hard negative samples. We further establish R^2 -HalBench, a new hallucination benchmark for MLLMs, which, unlike previous benchmarks, encompasses real-world, rich-context descriptions from 18 MLLMs with high-quality annotations, spanning diverse object-, attribute, and relationship-level details. VBackChecker outperforms prior complex frameworks and achieves state-of-the-art performance on R^2 -HalBench, even rivaling GPT-4o's capabilities in hallucination detection. It also surpasses prior methods in the pixel-level grounding task, achieving over a 10% improvement. All codes, data, and models are available at https://github.com/PinxueGuo/VBackChecker.

==> sec/3_method.tex <==
\section{Method}

\subsection{Verification by Visual Back Framework}

\paragraph{Problem Formulation. }
Our work addresses the problem of hallucination detection in Multimodal Large Language Models (MLLMs), which determines whether a given response from MLLMs contains visual hallucinations when conditioned on an input image. Specifically, let an MLLM $\Phi$ generate a descriptive response $R = \{r_1, r_2, \dots, r_n\}$ for an image $I$, where each rich-context sentence $r_i$ describes a specific visual part of the image: $ R = \Phi ( I ) $. 
Sentences $r_i$ may include visual hallucinations that conflict with the actual visual input, as the MLLMs rely on learned patterns rather than adhering to the visual information in $I$.
The goal of hallucination detection is to evaluate each $r_i$ and determine whether it contains a hallucination. This is formulated as a binary classification task for each $r_i$, where the label $y_i \in \{0, 1\}$ indicates the presence or absence of hallucinations. Specifically:
\begin{equation}
    y_i =
\begin{cases} 
0 & \text{if } r_i \text{ aligns with the visual input } I, \\
1 & \text{if } r_i \text{ conflicts with the visual input } I.
\end{cases}
\end{equation}

\begin{figure*}[ht]
    \centering
    \includegraphics[width=0.99\linewidth]{figures/figure_5_v3.pdf}
    \vspace{-2mm}
    \caption{
    \textbf{Visualization Results of Our \modelname{}}.
    Given the query tranformed from the response, \modelname{} employs a conversational model to predict either a [SEG] token or a [REJ] token to perform hallucination detection. Having a [SEG] token indicates that there is no hallucination, otherwise 
    \modelname{} outputs a [REJ] token and corresponding detailed explanation.
    } 
    \label{fig:result_visualization}
    \vspace{-2mm}
\end{figure*}


\paragraph{VBackChecker Framework. }
We propose the Verification by Vision Back Framework (\modelname{}), as illustrated in Fig.~\ref{fig:teaser}, to tackle this problem by leveraging a pixel-level Grounding LLM with reasoning and referring segmentation capabilities. The key idea behind \modelname{} is straightforward yet logical: Seeing is Believing. It verifies the response by “looking back” at the visual input.
For each $r_i$ in the MLLM's generated response, \modelname{} determines whether $r_i$ could be accurately grounded back to the input image $I$. If the grounding is successful, the sentence is free of hallucinations ($y_i = 0$); otherwise, it indicates the sentence contains a hallucination ($y_i = 1$).

\modelname{} employs a conversational model to predict either a [SEG] token or a [REJ] token to perform hallucination detection: When there is no hallucination in the MLLM's response $r_i$ based on the input image $I$, \modelname{} outputs a [SEG] token. 
The embedding of [SEG] before the LLM head is passed to a mask decoder (as in LISA~\cite{lai2023lisa}) to decode an object mask $m \in \mathbb{R}^{H \times W}$ corresponding to the described part in $r_i$. When the response $r_i$ contains a hallucination, \modelname{} outputs a [REJ] token and generates a detailed explanation in natural language indicating where $r_i$ conflicts with the visual content of $I$.
By combining pixel-level grounding and language-based reasoning, \modelname{} not only detects hallucinations but also provides interpretable outputs in both visual and language modalities. This dual capability ensures robust and reliable hallucination checking for MLLMs.  

However, existing Grounding LLMs lack the discriminative power for rich-context queries. While GSVA~\cite{Xia_2024_CVPR} attempts to reject references to non-existent objects, it struggles with fine-grained understanding. For example, when quering about a “... person in white” in an image with a person in black and a white wall, GSVA incorrectly predicts [SEG] instead of [REJ], failing to distinguish subtle attributes like object-specific colors. 



\begin{figure*}[ht]
    \centering
    \includegraphics[width=0.99\linewidth]{figures/figure_3_v3.pdf}
    \vspace{-2.5mm}
    \caption{
    A comprehensive analysis of our \ourbenchmark{} across four distinct dimensions.
    }
    \label{fig:bench}
    \vspace{-3mm}
\end{figure*}


\subsection{Instruct Data Generation}
\label{sec:instruct_data_generation}


To address this gap, we introduce Rich-context Instruct Tuning data (R-Insturct), built by the automated pipeline designed to generate high-quality rich-context visual instruction data for grounding and hallucination. 
R-Instruction includes grounding masks for positive queries and hallucination types with explanations for negative queries, ensuring both vision and language interpretability.



As illustrated in Figure~\ref{fig:pipeline}(a), we propose an automated four-step procedure to construct our R-Instruct data. 
Let $\mathcal{I}$ be the set of images sampled from the large-scale and high-quality SA1B dataset. For each image $I \in \mathcal{I}$: 

\newlength{\myDataSpace}
\setlength{\myDataSpace}{0.7mm}


\noindent\textbf{Object Proposal.} 
We first employ the Recognize Anything Model~\cite{ram} and the Grounded Segment Anything Model~\cite{gsam} to identify candidate objects $\{\Omega_m\}_{m=1}^{M}$, where each $\Omega_m$ includes a bounding box and a segmentation mask.

\noindent\textbf{Rich-context Caption.}
For each proposal $\Omega_m$, we employ Qwen2-VL-72B~\cite{wang2024qwen2} to generate a detailed caption $C_m$, capturing the category, shape, attributes (e.g., color, texture), spatial relationships, and distinctive features. This yields a set of object-description pairs, ensuring unique identification of objects within the image.

\noindent\textbf{Quality Control.}
To ensure accurate and diverse captions, by using CLIP~\cite{CLIP} and SBERT~\cite{reimers2019sentence}, we apply a multi-criteria filtering process:
(1) Foreground Background Check. 
Given a proposal {\small $\Omega_m$}, we compute CLIP scores for its foreground-masked image 
{\small $I_{\mathrm{fg}}^m$} 
and background-masked image 
{\small $I_{\mathrm{bg}}^m$}:
{\small $S_{\mathrm{fg}}^m = \mathrm{CLIP}(I_{\mathrm{fg}}^m, C_m)$,  $S_{\mathrm{bg}}^m = \mathrm{CLIP}(I_{\mathrm{bg}}^m, C_m)$}.
We retain captions where 
{\small $S_{\mathrm{fg}}^m > S_{\mathrm{bg}}^m$}
, ensuring the description aligns with the object rather than background artifacts.
(2) Vision-Text Consistency.
Captions with {\small $S_{\mathrm{fg}}^m$} below a confidence threshold (0.5) are discarded, filtering out poorly aligned descriptions.
(3) Multimodal Semantic NMS \textcolor{blue}{(Non-Maximum Suppression}. 
We propose a Multimodal Semantic NMS to remove near-duplicate proposals. We treat textual similarity $\mathrm{sim}(C_m, C_n)$ (computed via SBERT) as “semantic IoU” and use 
{\small $S_{\mathrm{fg}}^m$}
as a confidence score. Captions with high similarity to a higher-scoring reference are iteratively removed, ensuring each object retains its most coherent description.
This process yields $K$ high-quality samples $(\Omega_k, C_k)$, each with a precise mask and a verified rich-context caption.

\noindent\textbf{Hallucination Injection.}
To generate challenging negatives for hallucination detection, we prompt Qwen2-VL to perturb each valid caption $C_k$. Given the original image and descriptions of other objects in the scene, the model introduces misleading details—such as incorrect attributes or nonexistent objects—creating a hallucinated variant. Each hallucinated sample is annotated with its hallucination type (e.g., incorrect color, nonexistent object) and the corresponding explanation, ensuring the model is trained to accurately differentiate from misleading descriptions.

As shown in Figure~\ref{fig:pipeline}(b), we also collect holistic, multi-object captions (without per-object grounding masks) to better reflect real MLLM outputs. Using Claude-3.5, we generate comprehensive, rich-context descriptions covering all objects in an image, serving as additional positive samples. We then apply the same perturbation method to create corresponding negative samples.
As a result, the R-Instruct dataset comprises 30k images, 300k positive samples (100k with grounding masks), and 500k negative samples. Data from Figure~\ref{fig:pipeline}(a), which includes masks, is denoted R-Instruct-A, while data from Figure~\ref{fig:pipeline}(b), without masks, is R-Instruct-B. In positive samples, responses contain [SEG], whereas in negative samples, they include [REJ] with a hallucination explanation, as illustrated in Figure~\ref{fig:pipeline}(c).




\begin{figure*}[ht]
    \centering
    \includegraphics[width=0.99\linewidth]{figures/figure_4_v2.pdf}
    \vspace{-2mm}
    \caption{
    Samples of our \ourbenchmark.
    Each rich-context response, generated from various advanced MLLMs, is systematically annotated with corresponding hallucination categories.
    }
    \label{fig:bench_sample}
    \vspace{-2mm}
\end{figure*}




\subsection{Instruction Tuning}

The training methodology for Rich-context Instruction Tuning leverages a self-regressive learning framework tailored for multimodal grounding and hallucination detection. The overall loss function consists of two components: language loss ( $\mathcal{L}_L$ ) and grounding loss ( $\mathcal{L}_G$ ), defined as:

\begin{equation}
    \mathcal{L} = \mathcal{L}_L(t, t') + \mathcal{L}_G(m, m'),
\end{equation}



\noindent where  $t$  and  $m$  denote the predicted response and predicted mask, respectively, and  $t'$  and  $m'$  represent their corresponding ground truths. 
Specifically, $t = L_{\text{dec}}(h)$ , the textual output decoded by the language decoder  $L_{\text{dec}}$  from the hidden state  $h$.
{\small $m = G_{\text{dec}}(\text{MLP}(h[\text{SEG}]), I)$}, the predicted grounding mask generated by decoding the vision-guided hidden state  {\small $h[\text{SEG}]$}, processed through an MLP projector and conditioned on the image  $I $. $G_{\text{dec}}$ is the Mask Decoder, whose architecture follows that of SAM~\cite{SAM}.

The language loss $\mathcal{L}_L$ focuses solely on the response portion of the output sequence, evaluating the next-token prediction with Cross-Entropy Loss.
The grounding loss $\mathcal{L}_G$ employs a combination of per-pixel Binary Cross-Entropy Loss and DICE Loss to optimize the segmentation mask prediction.
Furthermore, unlike standard MLLM instruction tuning, where every output token equally contributes to the supervision signal, the performance of our grounding LLM, \modelname{}, hinges on its ability to make accurate predictions for the special tokens [SEG] and [REJ]. These tokens represent the model’s decision to either ground or reject a query and are crucial for hallucination detection. To emphasize their importance during training, we enhance their contributions to the loss function by applying higher weights to their Cross-Entropy terms. The modified language loss for these tokens is defined as:


\begin{equation}
    \footnotesize
    \mathcal{L}_L^{'} = -\sum \alpha_i \log P(t_i | t_{<i}),\; \\
    \alpha_i = 
    \begin{cases}
        \lambda,\! & \text{if } t_i \in \scriptstyle \{\text{[SEG]}, \text{[REJ]} \} \\
        1,\! & \text{otherwise}
    \end{cases}
\end{equation}


\noindent where $i$ indexes tokens in the response. $\lambda>1$ is a hyperparameter that amplifies the contributions of [SEG] and [REJ], guiding the model to emphasize learning critical decisions. 

==> tables/table_3_2.tex <==
\begin{table*}[htbp]

\newcommand{\greentick}{\Large\textcolor{green!70!black}{$\checkmark$}}
\newcommand{\redcross}{{\textcolor{red}{$\times$}}}

\centering
\normalsize

\scalebox{0.75}{
\begin{tabular}{cc|cc|cccccc|cccc}
\toprule

\multirow{4}{*}{\textbf{Evaluator}} &
\multirow{4}{*}{\textbf{LLM}} & 
\multicolumn{2}{c|}{\multirow{2}{*}{  \textbf{Explainability}}} &   
\multicolumn{6}{c|}{\multirow{2}{*}{  \textbf{HalMetaBench}} }  & 
\multicolumn{4}{c}{\multirow{2}{*}{  \textbf{POPE}}} \\

& &
\multicolumn{2}{c|}{} &   
\multicolumn{6}{c|}{} & 
\multicolumn{4}{c}{} \\

\cmidrule{3-4}\cmidrule{5-10}\cmidrule{11-14}


& & 
\multirow{2}{*}{\textbf{Visual}} & 
\multirow{2}{*}{\textbf{Text}} & 
\multirow{2}{*}{\textbf{Acc}} & 
\multicolumn{4}{c}{\textbf{NegAcc}} & 
\multirow{2}{*}{\textbf{PosAcc}} & 
\multicolumn{4}{c}{\textbf{Acc \wu{remove this row?}}} \\

\cline{6-9}\cline{11-14}

& & & & 
& \raisebox{-3pt}{\textbf{All}}  
& \raisebox{-3pt}{\textbf{Object}}
& \raisebox{-3pt}{\textbf{Attribute}}
& \raisebox{-3pt}{\textbf{Relation}}
&
& \raisebox{-3pt}{\textbf{All}}
& \raisebox{-3pt}{\textbf{Random Acc} }
& \raisebox{-3pt}{\textbf{Popular Acc} }
& \raisebox{-3pt}{\textbf{Adv Acc} } \\

\midrule

GPT-4o & - 
&  &  
& 63.9 & 31.4 & 37.5 & 23.9 & 18.6 & 93.9
& 96.6 & 87.4 & 85.0 \\

GPT-4 & - 
&  & \greentick
& 68.3 & 53.8 & 61.6 & 43.2 & 39.2 & 81.6
& 98.8 & 91.4 & 79.9 \\

LLaVA-OneVision & 7B
&  &  
& 47.9 & 98.8 & 98.9 & 98.8 & 98.5 & 0.9
& 93.0 & 85.6 & 36.6 \\

LLaVA-OneVision & 7B
&  & \greentick
& 48.0 & 99.1 & 98.5 & 99.9 & 99.9 & 0.9
& 99.2 & 89.1 & 34.9 \\

Qwen2VL & 7B
&  &  
& 47.7 & 76.4 & 75.6 & 77.3 & 78.4 & 21.2
& 71.9 & 68.2 & 42.7 \\

Qwen2VL & 7B
&  & \greentick
& 48.9 & 79.8 & 80.1 & 79.2 & 79.9 & 20.5
& 77.5 & 72.6 & 41.4 \\

Qwen2VL & 72B
&  &  
& 48.5 & 83.2 & 83.1 & 86.4 & 78.4 & 16.5
& 64.6 & 62.3 & 44.7 \\

Qwen2VL & 72B
&  & \greentick 
& 47.9 & 81.7 & 82.4 & 79.8 & 81.9 & 16.8
& 68.3 & 65.3 & 42.7 \\


& 
&  & 
&  &  &  &  &  & 
&  &  &  \\


GSVA & 7B
& \greentick &  
& 49.9 & 0.5 & 0.7 & 0.3 & 0.0 & 99.3
& 23.3 & 48.3 & 72.0 \\

GSVA & 13B
& \greentick &  
& 49.8 & 0.2 & 0.3 & 0.0 & 0.0 & 99.5
& 0.5 & 10.8 & 64.9 \\

FaithScore & 7B+13B+GPT-3.5
&  &  
& 59.3 & 75.3 & 76.7 & 73.7 & 71.5 & 44.6
& 82.7 & 83.0 & 78.9 \\

\rowcolor{gray!17} Ours & 7B
& \greentick & \greentick
& 62.5 & 64.1 & 64.2 & 63.4 & 64.9 & 60.9
& 99.3 & 93.2 & 70.3 \\







\bottomrule


\end{tabular}
} 

\caption{table 3}
\label{tab:main_results}
\end{table*}

==> tables/table_3_temp.tex <==


\begin{table*}[htbp]

\newcommand{\greentick}{\normalsize\textcolor{green!70!black}{$\checkmark$}}
\newcommand{\redcross}{{\textcolor{red}{$\times$}}}

\centering
\scriptsize
\renewcommand{\arraystretch}{1.15}

\begin{tabular}{cc|cc|cccccc|cccc}

\toprule

\multirow{3}{*}{\textbf{Evaluator}} &
\multirow{3}{*}{\textbf{LLM}} & 
\multicolumn{2}{c|}{\multirow{1}{*}{\textbf{Explainability}}} &   
\multicolumn{6}{c|}{\multirow{1}{*}{\textbf{HalMetaBench}}} & 
\multicolumn{4}{c}{\multirow{1}{*}{\textbf{POPE}}} \\


\cmidrule{3-4}\cmidrule{5-10}\cmidrule{11-14}

& & 
\multirow{2}{*}{\textbf{Visual}} & 
\multirow{2}{*}{\textbf{Text}} & 
\multirow{2}{*}{\textbf{Acc}} & 
\multicolumn{4}{c}{\textbf{NegAcc}} & 
\multirow{2}{*}{\textbf{PosAcc}} & 
\multicolumn{4}{c}{\textbf{Acc}} \\

\cline{6-9}\cline{11-14}

& & & & 
& \textbf{All} 
& \textbf{Object}
& \textbf{Attribute}
& \textbf{Relation}
&
& \textbf{All}
& \textbf{Random Acc} 
& \textbf{Popular Acc} 
& \textbf{Adv Acc} \\
\midrule


GPT-4o & -
& \greentick &
& 63.8 & & & &
& & & & \\

QwenZVL & 7B &  &  & & & & & & & & & & \\

QwenZVL & 72B &  &  & & & & & & & & & & \\

FaithScore & 7B+GPT &  &  & 59.3 & 75.3 & & & & 44.6 & & & & \\

GSVA & 7B & \greentick  &  & 49.9 & 0.5 & 0.7 & 0.3 & 0.0 & 99.3 & 62.2 & 23.3 & 48.3 & 72.0 \\

GSVA & 13B & \greentick  &  & 49.8 & 0.2 & 0.3 & 0.0 & 0.0 & 99.5 & 49.8 & 0.5 & 10.77 & 64.9 \\

\midrule

\rowcolor{gray!20} Ours & 7B & \greentick & \greentick & 62.5 & 64.1 & 64.2 & 63.4 & 64.9 & 60.9 & 76.9 & 99.3 & 93.22 & 70.3 \\

\bottomrule
\end{tabular}
\caption{Main Results}
\label{tab:main_results}
\end{table*}
